SimC3D: A Simple Contrastive 3D Pretraining Framework Using RGB Images

The 3D contrastive learning paradigm has demonstrated remarkable performance in downstream tasks through pretraining on point cloud data. Recent advances involve additional 2D image priors associated with 3D point clouds for further improvement. Nonetheless, these existing frameworks are constrained by the restricted range of available point cloud datasets, primarily due to the high costs of obtaining point cloud data. To this end, we propose SimC3D, a simple but effective 3D contrastive learning framework, for the first time, pretraining 3D backbones from pure RGB image data. SimC3D performs contrastive 3D pretraining with three appealing properties. (1) Pure image data: SimC3D simplifies the dependency of costly 3D point clouds and pretrains 3D backbones using solely RBG images. By employing depth estimation and suitable data processing, the monocular synthesized point cloud shows great potential for 3D pretraining. (2) Simple framework: Traditional multi-modal frameworks facilitate 3D pretraining with 2D priors by utilizing an additional 2D backbone, thereby increasing computational expense. In this paper, we empirically demonstrate that the primary benefit of the 2D modality stems from the incorporation of locality information. Inspired by this insightful observation, SimC3D directly employs 2D positional embeddings as a stronger contrastive objective, eliminating the necessity for 2D backbones and leading to considerable performance improvements. (3) Strong performance: SimC3D outperforms previous approaches that leverage ground-truth point cloud data for pretraining in various downstream tasks. Furthermore, the performance of SimC3D can be further enhanced by combining multiple image datasets, showcasing its significant potential for scalability. The code will be available at https://github.com/Dongjiahua/SimC3D.

==> fig/learning_obj.tex <==
\begin{figure*}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=1\textwidth, trim=25mm 45mm 30mm 70mm, clip]{fig/learning_obj_eccv.pdf}
\end{center} 
\vspace{-5mm}
\caption{\textbf{SimC3D Learning Objective Exploration}}
\vspace{-10pt}
\label{fig:obj}
\end{figure*}

==> fig/teaser.tex <==
\begin{figure*}[!htbp] % Adjusted placement specifiers
    \centering
    \includegraphics[width=\textwidth, trim=35mm 35mm 40mm 22mm]{fig/Teaser_3D.pdf}
    \caption{Your caption here}
    \label{fig:teaser}
\end{figure*}

==> tab/reduc_pos.tex <==
\begin{table}[t]
\vspace{-5mm}
\centering
\begin{minipage}{0.50\textwidth}

\centering
{\small
\setlength{\tabcolsep}{1mm}{

\begin{tabular}{l|cc|c}
\toprule
\multirow{2}{*}{2D model} & \multicolumn{1}{c}{SUN RGB-D}     \\ \cline{2-2} 
                                             & AP25 \\ \hline
            4 block                                 & 60.4     \\ %\hline
           2 block + output layer                                & 60.4     \\ %\hline
          1 block + output layer                                  &  60.1    \\ %\hline
             output layer                            & 60.3     \\ 
\bottomrule

\end{tabular}
% \vspace{-2mm}
\caption{\textbf{ResNet18 Reduction}: We gradually reduce the ResNet18 architecture to one simple convolutional layer. The performance is not lowered.}

\label{tab:reduc_layers}
}}
\end{minipage}
\hspace{3mm}
\begin{minipage}{0.45\textwidth}
% \begin{table}[h]
{\small
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{l|cc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{SUN RGB-D}  \\ \cline{2-3} 
                      &   AP50 & AP25    \\ \hline
From Scratch           &32.9 &57.7    \\ %\hline
Position Classification          & 35.0 & 60.2   \\ %\hline
Position Contrast                  & \textbf{36.2} &\textbf{61.2}   \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Position Learning Ablation.} Compared with the variant of position classification, Position contrast shows better performance}
\label{tab:pos_det}
}
}
\end{minipage}

\end{table}

==> tab/runtime.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|cc}
\small
\toprule
Model           & Total Params & One Iteration \\ \hline
3D SparseUNet   & 37.36M       & -                  \\
+ ViT           & 88.58M\oincrease{51.22M}       & 0.16s              \\
+ ResNet101     & 78.19M\oincrease{40.83M}       & 0.25s              \\
+ SimC3D (Ours) & 37.38M\myincrease{0.02M}       & 0.12s           \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\caption{\textbf{Training speed and Parameter numbers}}
\label{tab:runtime}
\vspace{-5mm}
\end{table}


==> tab/table_cluster2.tex <==
\begin{table*}[ht]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \begin{tabular}{c|cc|c}
        \toprule
        
        \multirow{2}{*}{2D model} & \multirow{2}{*}{trainable} & \multirow{2}{*}{pretrained} & \multicolumn{1}{c}{SUN RGB-D}     \\ \cline{4-4} 
                                  &                            &                             & AP25 \\ \hline
                    Vit-tiny     &\xmark                      &\cmark       &60.1\\ 
                    ResNet50       &  \xmark                        &    \cmark                            & 60.5     \\ %\hline
                   ResNet18       &  \xmark                        &    \cmark                            & 60.1     \\ %\hline
                  ResNet18       & \cmark                  &   \xmark                               &  60.4    \\ %\hline
                   ResNet18       &  \xmark                        &    \xmark                           & 60.1     \\ 
        \bottomrule
        
        \end{tabular}
        \caption{\textbf{Analysis of different backbones}: There's no significant difference between different backbones, even for the random initialized and frozen ResNet~\cite{resnet}.}
        \vspace{-5pt}
        \label{tab:reduc_models}
    \end{minipage}\hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \begin{tabular}{l|cc|c}
        \toprule
        \multirow{2}{*}{2D model} & \multicolumn{1}{c}{SUN RGB-D}     \\ \cline{2-2} 
                                                     & AP25 \\ \hline
                    4 block                                 & 60.4     \\ %\hline
                   2 block + output layer                                & 60.4     \\ %\hline
                  1 block + output layer                                  &  60.1    \\ %\hline
                     output layer                            & 60.3     \\ 
        \bottomrule
        
        \end{tabular}
        \caption{\textbf{ResNet18 Reduction}: We gradually simplify the ResNet18 architecture to one simple convolutional layer. The performance is not lowered.}
        \vspace{-5pt}
        \label{tab:reduc_layers}
    \end{minipage}\hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \begin{tabular}{l|cc}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c}{SUN RGB-D}  \\ \cline{2-3} 
                              &   AP50 & AP25    \\ \hline
        From Scratch           &32.9 &57.7    \\ %\hline
        Position Classification          & 35.0 & 60.2   \\ %\hline
        Position Contrast                  & \textbf{36.2} &\textbf{61.2}   \\ 
        \bottomrule
        \end{tabular}
        \caption{\textbf{Position Learning Ablation.} Compared with the variant of position classification, Position contrast shows better performance}
        \label{tab:pos_det}
    \end{minipage}


\end{table*}
